GPU Offloading in ExaHyPE Through C++ Standard Algorithms

The ISO C++17 standard introduces \emph{parallel algorithms}, a parallel programming model promising portability across a wide variety of parallel hardware including multi-core CPUs, GPUs, and FPGAs. Since 2019, the NVIDIA HPC SDK compiler suite supports this programming model for multi-core CPUs and GPUs. ExaHyPE is a solver engine for hyperbolic partial differential equations for complex wave phenomena. It supports multiple numerical methods including Finite Volumes and ADER-DG, and employs adaptive mesh refinement with dynamic load balancing via space-filling curves as well as task-based parallelism and offloading to GPUs. This study ports ExaHyPE's tasks over blocks of Finite Volumes to the ISO C++ parallel algorithms programming model, and compares its performance and usability against an OpenMP implementation with offloading via OpenMP target directives. It shows that ISO C++ is a feasible programming model for non-trivial applications like our task-based AMR code. The realisation is bare of vendor-specific or non-C++ extensions. It however is slower than its OpenMP counterpart. \vspace{-1cm}

==> 05_keywords.tex <==
\keywords{GPU, C++, ExaHyPE, hyperbolic PDE solvers} %% First letter not capped

